Continuous Space Reordering Models for Phrase-based MT

Bilingual sequence models improve phrase-based translation and reordering by overcoming phrasal independence assumption and handling long range reordering. However, due to data sparsity, these models often fall back to very small context sizes. This problem has been previously addressed by learning sequences over generalized representations such as POS tags or word clusters. In this paper, we explore an alternative based on neural network models. More concretely we train neuralized versions of lexicalized reordering and the operation sequence models using feed-forward neural network. Our results show improvements of up to 0.6 and 0.5 BLEU points on top of the baseline German->English and English->German systems. We also observed improvements compared to the systems that used POS tags and word clusters to train these models. Because we modify the bilingual corpus to integrate reordering operations, this allows us to also train a sequence-to-sequence neural MT model having explicit reordering triggers. Our motivation was to directly enable reordering information in the encoder-decoder framework, which otherwise relies solely on the attention model to handle long range reordering. We tried both coarser and fine-grained reordering operations. However, these experiments did not yield any improvements over the baseline Neural MT systems.

==> figure.tex <==
\begin{figure}%[htbp!]
\centering
\footnotesize
\begin{tikzpicture}[shorten >=1pt,->,draw=black!50, node distance=\layersep]
    \tikzstyle{every pin edge}=[<-]

	\tikzstyle{neuron}=[circle,fill=black!50,minimum size=20pt,inner sep=0pt]
	\tikzstyle{emb1}=[rectangle,fill=blue!100,minimum width=10pt, minimum height=25pt,inner sep=0pt]
	\tikzstyle{emb2}=[rectangle,fill=red!100,minimum width=10pt, minimum height=25pt,inner sep=0pt]
	\tikzstyle{plate}=[rectangle,draw=black!100,minimum width=50pt,minimum height=55pt,thin,inner sep=0pt]

	\tikzstyle{input neuron}=[neuron, fill=green!50];
    \tikzstyle{output neuron}=[neuron, fill=red!100];
    \tikzstyle{hidden neuron}=[neuron, fill=black];
    \tikzstyle{noise node}=[neuron, fill=gray!100];
    \tikzstyle{class node}=[neuron, fill=brown!100];

	\tikzstyle{annot} = [text width=4em, text centered]

    % Draw the input layer nodes
  %  \foreach \name / \y in {1,...,3}
  %      \node[emb1, pin=left:Source token \y] (I-\name) at (0,-\y) {};

	\node[emb1, pin=left:just] (I-1) at (0,-1) {};
	\node[emb1, pin=left:as ] (I-2) at (0,-2) {};
\node[emb1, pin=left: irresponsible] (I-3) at (0,-3) {};

	\node[emb1, pin=left: to] (I-4) at (0,-4) {};

    % Draw the hidden layer nodes
    \foreach \name / \y in {1,...,6}
        \path[yshift=0.5cm]
            node[hidden neuron] (H-\name) at (\layersep,-\y) {};

    % Draw the output layer node
    \node[output neuron] (O) at (5, -3.1){};

    % Draw the nce nodes
 %   \node[noise node] (N) at (7.0, -5.0){};
%    \node[class node] (C) at (7.0, -2.2){};
 %   \node[plate] (P) at (7, -5.1) {};

    % Draw the parameters nodes
%    \node[noise node] (NP) at (9.0, -5.0){};
%    \node[class node] (CP) at (9.0, -2.2){};

    % Connect every node in the input layer with every node in the
    % hidden layer.
    \foreach \source in {1,...,4}
        \foreach \dest in {1,...,6}
            \path (I-\source) edge (H-\dest);

    % Connect every node in the hidden layer with the output layer
    \foreach \source in {1,...,6}
        \path (H-\source) edge (O);

    % Connect the class node with noise and output layer
    %\path (C) edge (O);
    %\path (C) edge (N);
    %\path (NP) edge (N);
    %\path (CP) edge (C);

    % Annotate the layers
    \node[annot,above of=H-1, node distance=0.8cm] (hl) {Hidden layer};
    \node[annot,below of=H-6, node distance=0.8cm] {$\phi({\mathbf{x_n}})$};
    \node[annot,left of=hl] {Look-up layer};
    \node[annot,below of=I-4, node distance=0.7cm] {$\mathbf{x_n}$};
    \node[annot,right of=hl] {Output layer};
     \node[annot,below of=O, node distance=0.7cm]  {$\mathbf{y_n}$};
%    \node[annot,above of=C, node distance=0.6cm] {$C$};
%    \node[annot,left of=N, node distance=0.6cm, yshift=0.3cm] {$y_n^m$};
%    \node[annot,above of=O, node distance=0.6cm] {$y_n$};
%    \node[annot,below of=P, node distance=0.7cm, xshift=0.6cm] {$M$};
%    \node[annot,right of=H-2, node distance=1.3cm] {$\mathbf{W}$};
%    \node[annot,left of=H-1, node distance=1.3cm, yshift=0.1cm] {$\mathbf{U}$};
%    \node[annot,above of=NP, node distance=0.5cm] {$\psi$};
%    \node[annot,above of=CP, node distance=0.5cm] {$\pi$};    
\end{tikzpicture}
\caption{Neural OSM model where we use $3$-gram target words and a source context window of size $4$. For illustration, the output $y_n$ is shown as a single categorical variable (scalar) as opposed to the traditional one-hot vector representation.}
\vspace{-2mm}
\label{fig:NN}
\end{figure}
